Nanowire Melting Modes during the Solid-Liquid Phase Transition: Theory and Molecular Dynamics Simulations

Molecular dynamics simulation have shown that after initial surface melting, nanowires can melt via two mechanisms: an interface front moves towards the wire centre; the growth of an instability at the interface can cause the solid to pinch-off and breakup. By perturbing a capillary fluctuation model describing the interface kinetics, we show when each mechanism is preferred and compare the results to molecular dynamics simulation. A Plateau-Rayleigh-type of instability is found, and suggests longer nanowires will melt via a instability mechanism, whereas in shorter nanowires the melting front will move closer to the centre before the solid pinch-off can initiate. Simulations support this theory; preferred modes that destabilise the interface are proportional to the wire length, with longer nanowires preferring to pinch-off and melt; shorter wires have a more stable interface close to their melting temperature, and prefer to melt via an interface front that moves towards the wire centre.

==> Stb_Model.tex <==
\section{Allen-Cahn Model}
Melting at the nanoscale is thought to initiate at the surface, and then move from the outside inwards, with the interface consuming the solid as it melts. However, it has been observed in nanowires that as $T\rightarrow T_{\textrm{m}}$ the solid will begin to neck and breakup \cite{ridings2019surface}. In Figure~\ref{Fig:Melt_modes} a) we see a top-down view a nanowire at a temperature $T$ that sits between its surface melting temperature $T_{\textrm{s}}$ and bulk melting temperature $T_{\textrm{m}}$. Figure~\ref{Fig:Melt_modes} b) shows as $T \rightarrow T_{\textrm{m}}$ the solid is consumed as the interface moves towards the wire centre. Figure~\ref{Fig:Melt_modes} c) shows a side-on view of a the same nanowire. However, as $T \rightarrow T_{\textrm{m}}$, rather than the interface moving towards the centre, a portion of the solid begins to thin out and neck, initiating the breakup of the solid as seen in Figure~\ref{Fig:Melt_modes} d).
\begin{figure}[htp]
	\centering
{\includegraphics[width=0.4\textwidth]{Figures/Melting_modes.png}}
    \caption{Two different melting modes of nanowires where light grey represents the liquid, while the dark grey represents the solid. Panels a) to b) represent the moving interface front mechanism, whereas panels c) to d) show melting initiated via a instability at the solid-liquid interface.}
	\label{Fig:Melt_modes}   
\end{figure}
\\
To describe the observation in Figure~\ref{Fig:Melt_modes} d), a model for nanowire stability is made by taking a Allen-Cahn equation for a non-conserved order parameter to model the interface dynamics \cite{allen1979microscopic}. This involves perturbing a previously developed Landau-Ginzburg model to make it time-dependent \cite{ridings2019surface},
\begin{equation}
\label{Eq:Allen_Cahn}
\frac{\partial M}{\partial t} = \mu \frac{\delta F}{\delta M}.
\end{equation}
Here, $\mu$ is a diffusion-type of coefficient and $\frac{\delta F}{\delta M}$ is the functional derivative of the free energy in terms of an order parameter $M$ which takes the form $\frac{\delta F}{\delta M} = J \nabla^2 M - f'(M)$. Here $J = 4 \gamma_{\textrm{sl}} \xi$ with $\gamma_{\textrm{sl}}$ being the solid-liquid interfacial energy and $\xi$ is the correlation length. The bulk free energy of the system is $f(M)$ and is approximated as a pair of parabolas defined piecewise:
\begin{equation}
\label{Eq:bulk_FE}
f(M) = \begin{cases} 
\frac{\alpha}{2} M^2 + \Lambda(T) & \mbox{for } M < M^* \\
\frac{\alpha}{2} \left(1-M\right)^2 & \mbox{for } M > M^* \end{cases}. 	
\end{equation}
$\Lambda(T) =  L_{\textrm{v}} (1 - T/T_c)$ represents the difference in bulk free energy per unit volume between the solid and liquid phases at a temperature $T$, and $\alpha = 4\gamma_{\textrm{sl}}/\xi$ is a material dependent parameter\cite{pluis1990surface}. The intersection of the two parabolas defined in \Cref{Eq:bulk_FE} is $M^* = \frac{1}{2} - \frac{\Lambda(T)}{\alpha}$. 
We perturb the solid-liquid interface by a small parameter $\epsilon$, so we can express the solid-liquid interface as the surface $M[{r^*}(z,t)] = M^*$, where ${r}(z,t) = r^* + \epsilon e^{ikz + \omega t}$, with $r^*$ being the equilibrium radius of the solid during phase coexistence.
We take normal components of the order parameter $\nabla^2 M = \nabla^2_{\hat{n}} M + (\nabla \cdot \hat{n}) \nabla_{\hat{n}} M$, where $(\nabla \cdot \hat{n}) = R_1 + R_2 = \frac{1}{r^*}(1 + \frac{\epsilon}{r^*}(k^2(r^*)^2 - 1)e^{ikz + \omega t})$ and are the principal curvatures.
It can be shown that \Cref{Eq:Allen_Cahn} can be expressed as
\begin{equation}
\label{Eq:Allen-Cahn-Normal}
\frac{\partial M}{\partial t} =  \mu[J (\nabla^2_{{\hat{n}}} M + (R_1 + R_2) \nabla_{\hat{n}} M) - f'(M)],
\end{equation}
where $\nabla_{\hat{n}} M = \frac{\partial M}{\partial r} - \epsilon e^{ikz + \omega t} \frac{\partial M}{\partial z}$ and is the normal component of the order parameters gradient at the surface.
\begin{figure}[htp]
	\centering
{\includegraphics[width=0.5\textwidth]{Figures/Stab_Model2.png}}
    \caption{A surface melted nanowire of radius $R_0$ and length $L$. The solid core radius during solid-liquid phase coexistence is $r^*$. This surface has undergone a small perturbation in the form of a plane wave $r^* + \epsilon e^{ikz + \omega t}$. $M=M^*$ indicates the phase boundary, and the solid and liquid phases in the vicinity of the wire with $M>M^*$ and $M<M^*$ as indicated.}
	\label{Fig:Surf_Lin_melt}   
\end{figure}
Using the definition of $\nabla_{\hat{n}} M$ and neglecting $\mathcal{O}(\epsilon^2)$ terms we can expand  equation~\ref{Eq:Allen-Cahn-Normal} to get
\begin{multline}
\label{Eq:Allen-Cahn-Normal_2}
\frac{\partial M}{\partial r}\frac{\partial r}{\partial t} =  \mu[J (\frac{\partial ^2 M}{\partial r^2} + \frac{1}{r^*}(1 + \frac{\epsilon}{r^*}(k^2(r^*)^2 -\\
1)e^{ikz + \omega t}) \frac{\partial M}{\partial r}) - \alpha(1-M)].
\end{multline}
One can see by solving equation~\ref{Eq:Allen-Cahn-Normal_2} to $\mathcal{O}(1)$ we recover the solution to $\frac{\delta F}{\delta M}=0$. Solving equation~\ref{Eq:Allen-Cahn-Normal_2} to $\mathcal{O}(\epsilon)$ we arrive at the dispersion relation for the solid profile of the coexisting nanowire
\begin{equation}
    \label{Eq:omega}
\omega = \frac{\mu J}{(r^*)^2}(1 - k^2(r^*)^2).
\end{equation}
A PR type instability can be found by observing that $\omega > 0$ when $kr^* < 1$, bringing us to the familiar solution
\begin{equation}
    \label{Eq:PR_Stability}
\lambda^* >   2 \pi r^*.
\end{equation}
Classical nucleation theory tells us that Gibbs free energy difference in an infinitely long crystal cylinder of radius $r$ surrounded by its own melt near the melting temperature can be expressed as \cite{wu2015self} 
\begin{equation}
    \label{Eq:CNT_Cylinder}
\Delta G = - \pi r^2  L_{\textrm{v}}(\Delta T/T_c)+ 2 \pi r \gamma_{\textrm{sl}}.
\end{equation}
Finding the value of $r$ that minimizes this equation gives the solution 
\begin{center}
\begin{equation}
    \label{Eq:CNT_rstar}
r^* =  \frac{\gamma_{\textrm{sl}}T_c}{ L_{\textrm{v}} \Delta T}.
\end{equation}
\end{center}
We combine equations~\ref{Eq:PR_Stability} and \ref{Eq:CNT_rstar} and take $\Delta T = T_c - T_{\textrm{m}}$, where $T_\textrm{m}$ is the bulk melting temperature of a nanowire of radius $R_0$. The interface will remain stable when $\omega < 0$ and leads  to the moving interface front seen in Figure~\ref{Fig:Melt_modes} a) to b) giving the condition
\begin{center}
\begin{equation}
    \label{Eq:T_omega}
T_{\omega} < T_{\textrm{m}},
\end{equation}
\end{center}
where we define $T_{\omega}=T_c\bigg(1 - \frac{2 \pi \gamma_{\textrm{sl}}}{ L_{\textrm{v}} \lambda^*}\bigg)$. For $\omega > 0$ we have $ T_{\omega} > T_{\textrm{m}}$, and perturbations will grow to destabilise the solid-liquid interface, giving the scenario in Figure~\ref{Fig:Melt_modes} c) to d). If $\lambda^* \propto L$ then $T_{\omega}$ becomes larger than $T_{\textrm{m}}$ quickly, giving a clear criteria for describing when each melting mode is preferred.
\\
Finally, by combining equations~\ref{Eq:CNT_rstar} and $T_{\textrm{m}}$ from previous work \cite{ridings2019surface}, a equation for the equilibrium solid radius $r^*$ in terms of initial wire radius $R_0$ and interfacial energies $\kappa$ (where $\kappa = \frac{1-\Delta \gamma /\gamma_{\textrm{sl}}}{1+\Delta \gamma /\gamma_{\textrm{sl}}}$ and $\Delta \gamma$ is the spreading parameter that determines the wettability of a material \cite{ridings2019surface})
\begin{center}
    \begin{equation}
    \label{Eq:rstar_R0}
    r^* = \frac{R_0}{4}\bigg( \kappa +  \frac{I_0(R_0/\xi)}{I_1(R_0/\xi)} \bigg),
\end{equation}
\end{center}
which shows how the equilibrium solid radius scales with size. 
